Understanding the atmospheric properties and chemical composition of the ultra-hot Jupiter HAT-P-7b II. Mapping the effects of gas kinetics

The atmospheres of ultra-hot Jupiters are commonly considered to be at thermochemical equilibrium. We aim to provide disequilibrium chemistry maps for a global understanding of the chemistry in HAT-P-7b's atmosphere and assess the importance of disequilibrium chemistry on UHJs. We apply a hierarchical modelling approach utilising 97 1D atmospheric profiles from 3D GCM of HAT-P-7b. For each 1D profile, we evaluate our kinetic cloud formation model consistently with the local gas-phase composition in chemical equilibrium. We then evaluate quenching results from a zeroth-order approximation in comparison to a kinetic gas-phase approach. We find that the zeroth-order approach of estimating quenching points agrees well with the full gas-kinetic modeling results. Chemical disequilibrium has the greatest effect on the nightside and morning abundance of species such as H, H$_2$O, CH$_4$, CO$_2$, HCN, and all C$_n$H$_m$ molecules; heavier C$_n$H$_m$ molecules are more affected by disequilibrium processes. CO abundance, however, is affected only marginally. While dayside abundances also notably change, those around the evening terminator of HAT-P-7b are the least affected by disequilibrium processes. The latter finding may partially explain the consistency of observed transmission spectra of UHJs with atmospheres in thermochemical equilibrium. Photochemistry only negligibly affects molecular abundances and quenching levels. In general, the quenching points of HAT-P-7b's atmosphere are at much lower pressures in comparison to the cooler hot-jupiters. We propose several avenues to look for the effect of disequilibrium processes on UHJs that are, in general, based on abundance and opacity measurements at different local times. It remains a challenge to completely disentangle this from the chemical effects of clouds and that of a primordial non-solar abundance.

==> HAT-p-7b%20Cloud%20mapping%3A%20gas-kinetics%20(rev1)%20(Arxiv_red_size)/tab_syspar.tex <==
% \documentclass{aastex}
% \begin{document}
\begin{table*}
\caption{Derived system parameters for the HAT-P-7 system}
\label{table:comparison}
\centering                      
\begin{tabular}{c c c }     
\hline\hline                
% \hline 
Orbital Parameters & & \\
\hline\hline 
Period~ $P$	~(days)							 		  & 2.204735471 $\pm$ 0.0000024				&   \citet{masuda15} 	\\
Eccentricity~ $e$								      &	0.0										& 	\citet{pal08}	    \\
Inclination~ $i$ (degrees)						      & 86.68 $\pm$ 0.14						&	\citet{vaneylen13}   \\
Semi-major axis~ $a$ ~(AU)							  & 0.0379 $\pm$ 0.0004						& 	\citet{pal09}	    \\
\hline\hline 
Stellar Parameters & & \\
\hline\hline  
Stellar mass~ $M_{\star} ~(M_{\odot})$       	  	  & 1.36 $\pm$ 0.02 						&	\citet{vaneylen13}   \\
Stellar radius~ $R_{\star} ~(R_{\odot})$  	 	  	  & 1.90 $\pm$ 0.01  					    &  	\citet{vaneylen13} 	 \\
Surface gravity~ $log(g_{\star})$ ~(cgs)	 	  	  & 4.01 $\pm$ 0.01 						& 	\citet{vaneylen13}   \\
Stellar Temperature~ $T_{eff} ~(K)$     	 	  	  & 6259 $\pm$ 32 							&   \citet{vaneylen13} 	 \\
Metallicity~ $[Fe/H]$          			     	  	  & $+$0.26 $\pm$ 0.08						& 	\citet{pal08} 	     \\
\hline\hline 
Planetary Parameters & & \\
\hline\hline 
Planetary mass~ $M_{p}$ ($M_{\rm Jup}$) 			  & 1.74 $\pm$ 0.03 	  	    		    & 	\citet{vaneylen13}   \\
Planetary radius~ $R_{p}$ ($R_{\rm Jup}$) 			  & 1.43 $\pm$ 0.01    					    & 	\citet{vaneylen13}	 \\
Equibilibrium temperature~ $T_{\rm eq}$ (K)   		  &	2139 $\pm$ 27     					    &   \citet{heng13}	   \\
\hline\hline                                 
\end{tabular}
\end{table*}
% \end{document}



==> tab_syspar.tex <==
% \documentclass{aastex}
% \begin{document}
\begin{table*}
\caption{Derived system parameters for the HAT-P-7 system}
\label{table:comparison}
\centering                      
\begin{tabular}{c c c }     
\hline\hline                
% \hline 
Orbital Parameters & & \\
\hline\hline 
Period~ $P$	~(days)							 		  & 2.204735471 $\pm$ 0.0000024				&   \citet{masuda15} 	\\
Eccentricity~ $e$								      &	0.0										& 	\citet{pal08}	    \\
Inclination~ $i$ (degrees)						      & 86.68 $\pm$ 0.14						&	\citet{vaneylen13}   \\
Semi-major axis~ $a$ ~(AU)							  & 0.0379 $\pm$ 0.0004						& 	\citet{pal09}	    \\
\hline\hline 
Stellar Parameters & & \\
\hline\hline  
Stellar mass~ $M_{\star} ~(M_{\odot})$       	  	  & 1.36 $\pm$ 0.02 						&	\citet{vaneylen13}   \\
Stellar radius~ $R_{\star} ~(R_{\odot})$  	 	  	  & 1.90 $\pm$ 0.01  					    &  	\citet{vaneylen13} 	 \\
Surface gravity~ $log(g_{\star})$ ~(cgs)	 	  	  & 4.01 $\pm$ 0.01 						& 	\citet{vaneylen13}   \\
Stellar Temperature~ $T_{eff} ~(K)$     	 	  	  & 6259 $\pm$ 32 							&   \citet{vaneylen13} 	 \\
Metallicity~ $[Fe/H]$          			     	  	  & $+$0.26 $\pm$ 0.08						& 	\citet{pal08} 	     \\
\hline\hline 
Planetary Parameters & & \\
\hline\hline 
Planetary mass~ $M_{p}$ ($M_{\rm Jup}$) 			  & 1.74 $\pm$ 0.03 	  	    		    & 	\citet{vaneylen13}   \\
Planetary radius~ $R_{p}$ ($R_{\rm Jup}$) 			  & 1.43 $\pm$ 0.01    					    & 	\citet{vaneylen13}	 \\
Equibilibrium temperature~ $T_{\rm eq}$ (K)   		  &	2139 $\pm$ 27     					    &   \citet{heng13}	   \\
\hline\hline                                 
\end{tabular}
\end{table*}
% \end{document}


